List H-Coloring a Graph by Removing Few Vertices

In the deletion version of the list homomorphism problem, we are given graphs G and H, a list L(v) that is a subset of V(H) for each vertex v of G, and an integer k. The task is to decide whether there exists a subset W of V(G) of size at most k such that there is a homomorphism from G \ W to H respecting the lists. We show that DL-Hom(H), parameterized by k and |H|, is fixed-parameter tractable for any (P6, C6)-free bipartite graph H; already for this restricted class of graphs, the problem generalizes Vertex Cover, Odd Cycle Transversal, and Vertex Multiway Cut parameterized by the size of the cutset and the number of terminals. We conjecture that DL-Hom(H) is fixed-parameter tractable for the class of graphs H for which the list homomorphism problem (without deletions) is polynomial-time solvable; by a result of Feder, Hell and Huang (1999), a graph H belongs to this class precisely if it is a bipartite graph whose complement is a circular arc graph. We show that this conjecture is equivalent to the fixed-parameter tractability of a single fairly natural satisfiability problem, Clause Deletion Chain-SAT.

==> abstract.tex <==

\begin{abstract}
  In the deletion version of the list homomorphism problem for a fixed
  graph $H$ (\dlhom), we are given a graph $G$, a list $L(v)\subseteq
  V(H)$ for each vertex $v\in V(G)$, and an integer $k$, the task is
  to decide whether there exists a set $W \subseteq V(G)$ of size at
  most $k$ such that there is a homomorphism from $G\setminus W$ to
  $H$ respecting the lists. We show that \dlhom is fixed-parameter
  tractable for any $(P_6,C_6)$-free bipartite graph $H$; already for
  this restricted class of graphs, the problem generalizes Vertex
  Cover, Multiway Cut, and Odd Cycle Transversal. We conjecture that
  \dlhom is fixed-parameter tractable for the class of graphs $H$ for
  which the list homomorphism problem (without deletions) is
  polynomial-time solvable; by a result of Feder et
  al.~\cite{FederHH03}, a graph $H$ belongs to this class precisely if
  it is a bipartite graph whose complement is a circular arc graph. We
  show that this conjecture is equivalent to the fixed-parameter
  tractability of a single fairly natural satisfiability problem,
  \emph{Clause Deletion Chain-SAT}.
\end{abstract}



